Probe Before You Preach: Conformal Ambiguity Sets and Neuro-Symbolic Counterfactual Probing for Diagnosing Algebraic Misconceptions in Middle School Mathematics

Distinct mathematical misconception rules can produce the same incorrect answer, making diagnosis from a single response ambiguous. We formalize this algebraic collision and derive a conditional Bayes error bound; internally generated reasoning does not add student-specific information beyond its inputs under an explicit conditional-independence assumption. We propose Mondrian Adaptive Conformal Misconception Sets (MACMS) and Symbolic-Verified Counterfactual Micro-Probing (Sym-EIG). MACMS has curriculum-group marginal coverage under exchangeability, not a per-student correctness guarantee. Sym-EIG searches for probes whose outputs separate modeled candidate rules; identification additionally depends on the candidate set and response model. An audit of a local public Eedi graph finds 2,118 of 2,258 linked constructs associated with at least two misconception IDs; construct-level associations alone do not establish same-answer collisions. Other project performance tables require recomputation because their script assigns numerical results directly. No diagnostic performance or classroom learning benefit is claimed here. A classroom study is proposed for future validation.

==> tex/compat.tex <==
%% Journal compatibility layer.
%% jmp.cls already provides fonts, amsmath, amsthm, csquotes, hyperref,
%% and biblatex-chicago. Other classes get portable fallbacks so the same
%% metadata commands and citation macros still compile.

\makeatletter
\@ifclassloaded{jmp}{%
  %% JMP: nothing extra. Metadata commands and biblatex are already defined.
}{%
  \RequirePackage{amsmath}
  \RequirePackage{amssymb}
  \RequirePackage{amsthm}
  \RequirePackage{xcolor}
  \RequirePackage[style=american]{csquotes}
  \RequirePackage[font=small,labelfont=bf]{caption}
  \RequirePackage{graphicx}
  \RequirePackage{algorithm}
  \RequirePackage{algpseudocode}
  \RequirePackage[colorlinks=true,allcolors=blue]{hyperref}

  \@ifundefined{issueinfo}{\newcommand{\issueinfo}[1]{}}{}
  \@ifundefined{pubyear}{\newcommand{\pubyear}[1]{}}{}
  \@ifundefined{articledoi}{\newcommand{\articledoi}[1]{}}{}
  \@ifundefined{copyrightholders}{\newcommand{\copyrightholders}[1]{}}{}
  \@ifundefined{shorttitle}{\newcommand{\shorttitle}[1]{}}{}
  \@ifundefined{shortauthors}{\newcommand{\shortauthors}[1]{}}{}
  \@ifundefined{journalname}{\newcommand{\journalname}[1]{}}{}

  \@ifundefined{addauthor}{%
    \newif\ifpaper@hasauthor
    \newcommand{\addauthor}[4][]{%
      \ifpaper@hasauthor
        \g@addto@macro\@author{\and #2\thanks{#3；\texttt{#4}}}%
      \else
        \paper@hasauthortrue
        \author{#2\thanks{#3；\texttt{#4}}}%
      \fi
    }%
  }{}
}

\@ifundefined{definecolor}{\RequirePackage{xcolor}}{}
\definecolor{jmpinkiii}{HTML}{8C8474}
\makeatother


==> tex/preamble.tex <==
%% Shared packages and bibliography. Theorem names stay in each main file
%% so English and Chinese can use different headings.

\usepackage[margin=2.4cm]{geometry}
\usepackage{bm}
\emergencystretch=2em
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{array}
\usepackage{makecell}
\usepackage{enumitem}

\makeatletter
\@ifpackageloaded{biblatex}{}{%
  \RequirePackage[backend=biber,style=numeric,natbib=true]{biblatex}}
\makeatother
\addbibresource{refs.bib}
\setcounter{biburllcpenalty}{7000}
\setcounter{biburlucpenalty}{7000}
\setcounter{biburlnumpenalty}{7000}

\graphicspath{{figures/}}
\captionsetup[table]{position=top}
\usepackage{thm-restate}
\usepackage{booktabs}
\usepackage{tikz}
\usepackage{listings}
\lstset{basicstyle=\footnotesize\ttfamily,breaklines=true,breakindent=0pt,
  postbreak=\mbox{\textcolor{jmpinkiii}{$\hookrightarrow$}\space}}

%% 摘要：正文紧跟标签，不单独成行；下一行是关键词：
\makeatletter
\renewcommand{\abstractname}{\ifzh 摘要\else Abstract\fi}
\renewenvironment{abstract}{%
  \par\addvspace{1.25em}%
  \noindent\textbf{\abstractname\ifzh ：\else: \fi}%
  \ignorespaces
}{%
  \par
}
\newcommand{\keywords}[1]{%
  \par\noindent\textbf{\ifzh 关键词\else Keywords\fi\ifzh ：\else: \fi}#1\par
  \ifzh\else\addvspace{1.25em}\fi
}
%% 中文稿另附英文摘要、关键词（国内期刊常见）
\newenvironment{enabstract}{%
  \par\addvspace{0.85em}%
  \par\begingroup\centering\large\entitle\par\endgroup\vspace{0.45em}%
  \noindent\textbf{Abstract: }%
  \ignorespaces
}{%
  \par
}
\newcommand{\enkeywords}[1]{%
  \par\noindent\textbf{Keywords: }#1\par
  \addvspace{1.25em}%
}

\newcommand{\papermeta}{%
  \begingroup
    \def\@thefnmark{*}%
    \long\def\@makefntext##1{\par\noindent ##1}%
    \footnotetext{%
      \ifzh 收稿日期：\received；修回日期：\revised
      \else Received: \received; revised: 2026-11-04
      \fi
    }%
  \endgroup
}

\newenvironment{funding}
  {\par\addvspace{0.9em}\noindent\textbf{\ifzh 基金项目\else Funding\fi\ifzh ：\else: \fi}\ignorespaces}
  {\par}
\newenvironment{acknowledgments}
  {\par\addvspace{0.9em}\noindent\textbf{\ifzh 致谢\else Acknowledgments\fi\ifzh ：\else: \fi}\ignorespaces}
  {\par}
\newenvironment{conflictsofinterest}
  {\par\addvspace{0.9em}\noindent\textbf{\ifzh 利益冲突\else Conflicts of interest\fi\ifzh ：\else: \fi}\ignorespaces}
  {\par}

\ifzh
  \floatname{algorithm}{算法}
  \algrenewcommand\algorithmicrequire{\textbf{输入：}}
  \algrenewcommand\algorithmicensure{\textbf{输出：}}
\else
  \algrenewcommand\algorithmicrequire{\textbf{Input:}}
  \algrenewcommand\algorithmicensure{\textbf{Output:}}
\fi

%% ctex 中文方案默认将 section/part 居中；各级章节标题一律左对齐
\ifzh
  \ctexset{
    part/format         = \Large\bfseries\raggedright,
    section/format      = \Large\bfseries\raggedright,
    subsection/format   = \large\bfseries\raggedright,
    subsubsection/format= \normalsize\bfseries\raggedright,
    paragraph/format    = \normalsize\bfseries\raggedright,
    subparagraph/format = \normalsize\bfseries\raggedright,
  }
\fi
\makeatother
\usepackage{longtable}

